Markpainting: Adversarial Machine Learning meets Inpainting

Inpainting is a learned interpolation technique that is based on generative modeling and used to populate masked or missing pieces in an image; it has wide applications in picture editing and retouching. Recently, inpainting started being used for watermark removal, raising concerns. In this paper we study how to manipulate it using our markpainting technique. First, we show how an image owner with access to an inpainting model can augment their image in such a way that any attempt to edit it using that model will add arbitrary visible information. We find that we can target multiple different models simultaneously with our technique. This can be designed to reconstitute a watermark if the editor had been trying to remove it. Second, we show that our markpainting technique is transferable to models that have different architectures or were trained on different datasets, so watermarks created using it are difficult for adversaries to remove. Markpainting is novel and can be used as a manipulation alarm that becomes visible in the event of inpainting.

==> images/corresponding_result_table_images.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/results/aqueduct_eps0.1.png}
        \caption{Attacking RN.}
        \label{fig:aqueduct}
    \end{subfigure}%
    \begin{subfigure}{.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/results/aqueduct_combined_eps0.1.png}
        \caption{Attacking all models.}
        \label{fig:aqueduct_combined}
    \end{subfigure}
    \caption{Example outputs of the images used for evaluation and creation of~\Cref{tab:single_model} and~\Cref{tab:all_model}. Both images show output at $\epsilon=0.1$. Original image from Places2.}
\end{figure}

==> images/defences/defence2.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/defences/l2_target_2.png}
    \caption{Effect of different transformations to counter markpainting, measured by L2. \todo{Ilia: add new results}}
    \label{fig:defence2}
\end{figure}


==> images/results/eval_images.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{images/results/eval_images.png}
    \caption{Images to be used for evaluation. All the photos, other than the bottom-right window pane image, are original works of the Authors. The window image is taken from \href{https://zenwindowsnashville.com/should-you-add-window-grids-to-your-home-windows-a-modern-guide/}{ZenWindows}.}
    \label{fig:eval_images}
\end{figure}


==> images/self_encoding.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/self_encoding.png}
    \caption{Self-encoded images. Picture depicts artist Seamus Wray. Model was attacked for 500 iterations, with an $\epsilon=0.3$.}
    \label{fig:self_encoding}
\end{figure*}

==> tables/results_compact.tex <==

\begin{table*}[t]
% \centering
\begin{adjustbox}{scale=0.9,center}
\begin{tabular}{@{}llrrrr|rrrr|rrrr@{}}
\toprule
\multicolumn{2}{l}{Distance to:} &\multicolumn{4}{c|}{Original} & \multicolumn{4}{c|}{Adversarial Target} & \multicolumn{4}{c}{Benign} \\
$\epsilon$ & &Loss & $l_2$ & PSNR & SSIM & Loss & $l_2$ & PSNR & SSIM & Loss & $l_2$ & PSNR & SSIM\\
\midrule
\multirow{5}{*}{$ 0.0 $}
&GENERATIVE & 0.467 & 0.111 & 12.491 & 0.250 & 0.755 & 1.186 & -0.622 & 0.036 & 0.179 & 0.000 & 134.217 & 1.000\\
&RFR & 0.279 & 0.027 & 19.156 & 0.387 & 0.433 & 0.292 & 5.464 & 0.090 & 0.001 & 0.000 & 144.923 & 1.000\\
&RN & 0.300 & 0.025 & 17.891 & 0.420 & 0.473 & 0.292 & 5.438 & 0.104 & 0.001 & 0.000 & inf & 1.000\\
&CRFILL & 0.470 & 0.109 & 13.342 & 0.319 & 0.796 & 1.205 & -0.683 & 0.044 & 0.180 & 0.000 & inf & 1.000\\
&GMCNN & 0.485 & 0.122 & 10.891 & 0.210 & 0.721 & 1.136 & -0.432 & 0.047 & 0.181 & 0.000 & inf & 1.000\\
&EDGE CONNECT & 0.290 & 0.025 & 18.198 & 0.390 & 0.422 & 0.299 & 5.383 & 0.104 & 0.001 & 0.000 & 135.041 & 1.000\\
\midrule
\multirow{5}{*}{$ 0.03 $}
&GENERATIVE & 0.466 & 0.110 & 12.551 & 0.245 & 0.748 & 1.175 & -0.579 & 0.036 & 0.214 & 0.005 & 26.037 & 0.829\\
&RFR & 0.287 & 0.028 & 18.593 & 0.362 & 0.416 & 0.282 & 5.617 & 0.088 & 0.032 & 0.001 & 30.462 & 0.948\\
&RN & 0.361 & 0.065 & 12.642 & 0.294 & 0.266 & 0.194 & 7.520 & 0.214 & 0.231 & 0.043 & 14.735 & 0.497\\
&CRFILL & 0.472 & 0.107 & 13.200 & 0.299 & 0.786 & 1.180 & -0.589 & 0.044 & 0.230 & 0.008 & 23.472 & 0.809\\
&GMCNN & 0.484 & 0.121 & 10.816 & 0.206 & 0.717 & 1.129 & -0.405 & 0.048 & 0.195 & 0.005 & 31.205 & 0.922\\
&EDGE CONNECT & 0.291 & 0.025 & 18.041 & 0.378 & 0.407 & 0.293 & 5.489 & 0.107 & 0.036 & 0.001 & 29.890 & 0.911\\
\midrule
\multirow{5}{*}{$ 0.3 $}
&GENERATIVE & 0.487 & 0.115 & 11.625 & 0.169 & 0.734 & 1.099 & -0.270 & 0.025 & 0.312 & 0.036 & 16.181 & 0.400\\
&RFR & 0.373 & 0.043 & 14.869 & 0.215 & 0.374 & 0.211 & 6.988 & 0.076 & 0.191 & 0.022 & 17.416 & 0.633\\
&RN & 0.456 & 0.154 & 8.620 & 0.216 & 0.067 & 0.049 & 14.125 & 0.322 & 0.365 & 0.140 & 8.970 & 0.315\\
&CRFILL & 0.541 & 0.157 & 9.376 & 0.133 & 0.710 & 0.895 & 0.642 & 0.063 & 0.439 & 0.106 & 10.830 & 0.247\\
&GMCNN & 0.493 & 0.127 & 10.359 & 0.173 & 0.712 & 1.095 & -0.257 & 0.046 & 0.236 & 0.014 & 21.002 & 0.664\\
&EDGE CONNECT & 0.334 & 0.036 & 15.416 & 0.282 & 0.373 & 0.259 & 6.092 & 0.106 & 0.153 & 0.018 & 18.638 & 0.586\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Attack example related statistics with only RN model attacked. Here `Original' refers to the original image (\imagein) i.e. before a mask is applied, `Adversarial target' is the target image used in the optimization (\imagetarget), and `Benign' is the image that the inpainting model would have produced without any adversarial perturbation (\imagebenign). Calculations are performed only over the masked area. The results are after 100 iterations with a step size of $\frac{\epsilon}{50}$. A visual representation of the attack is shown in Appendix. Details are discussed in \Cref{sec:eval:transfer}.}
\label{tab:single_model_compact}
\end{table*}

